DexLego: Reassembleable Bytecode Extraction for Aiding Static Analysis

The scale of Android applications in the market is growing rapidly. To efficiently detect the malicious behavior in these applications, an array of static analysis tools are proposed. However, static analysis tools suffer from code hiding techniques like packing, dynamic loading, self modifying, and reflection. In this paper, we thus present DexLego, a novel system that performs a reassembleable bytecode extraction for aiding static analysis tools to reveal the malicious behavior of Android applications. DexLego leverages just-in-time collection to extract data and bytecode from an application at runtime, and reassembles them to a new Dalvik Executable (DEX) file offline. The experiments on DroidBench and real-world applications show that DexLego correctly reconstructs the behavior of an application in the reassembled DEX file, and significantly improves analysis result of the existing static analysis systems.

==> paragraphs/motivation.tex <==
\section{Motivation}
\label{sec:motivation}

As metioned in Section~\ref{sec:intro}, the method-level collection can not provide
a precise result on advanced self-modifying code. Take Code~\ref{lst:smc} as an 
example. While entering the method \texttt{leak}, its smali code is represented
by Code~\ref{lst:el}. After the first execution of the method \texttt{bytecodeTamper}, 
the code is modified to Code~\ref{lst:fe}. Next, the second execution of the native 
method resume the code back to Code~\ref{lst:el}. The 
length of instruction \texttt{invoke-virtual}, \texttt{move-result-object}, \texttt{const-string}, 
and \texttt{nop} are $6$ bytes, $2$ bytes, $4$ bytes, and $2$ bytes, respectively, and we add
two \texttt{nop} instructions in Code~\ref{lst:fe} to make the total length of the code unchanged.

The method-level solutions collects the code of method \texttt{leak} as a whole. 
DexHunter~\cite{dexhunter:esorics15} dumps the DEX file in the memory after
the class initialization and AppSpear~\cite{appspear:raid15} collects information 
after the activity \texttt{Main} is launched. However, both of them can only collect 
Code~\ref{lst:el}. Though AppSpear involves multiple collections and traces the 
method \texttt{leak} for multiple times, it still can only collect Code~\ref{lst:el}
as the second execution of the native method has resumed the code back to Code~\ref{lst:el}.
Further, the code of method \texttt{leak} in memory is either Code~\ref{lst:el} or \ref{lst:fe} at any time point, which means that any method-level collection could only collect either or both
of them from memory. Firstly, the \texttt{leak} method invokes both the method \texttt{normal}
and the method \texttt{sink}, so neither Code~\ref{lst:el} nor \ref{lst:fe} could represent the
actual behavior of the application alone. Secondly, as the Line $2$ of Code~\ref{lst:fe} is never executed, simply combining the two codes together does not work. 

In conclusion, the method-level solutions simplifies the collection phase, however, it could not 
precisely identify the actual behavior of advanced self-modifying code like Code~\ref{lst:smc}.
\TheName{} collects each executing instruction and reassembles all the collected instructions
back to a new DEX file. As all the collected instructions are actual executing instructions, the
new DEX file represents the behavior the application precisely.

\begin{lstlisting}[caption={This smali code represents the method \texttt{leak} while entering and leaving it.},label={lst:el}, language=Ant]
.method public leak()V
  <@\textcolor{red}{invoke-virtual { p0 }, \textbackslash}@>
  <@\ \ \textcolor{red}{Lcom/test/Main;->getSensitiveData()Ljava/lang/String;}@>
  <@\textcolor{red}{move-result-object v0}@>
  const/4 v1, 0
  :L0
  const/4 v2, 2
  if-ge v1, v2, :L1
  <@\textcolor{blue}{invoke-virtual { p0, v0 }, \textbackslash}@>
  <@\ \ \textcolor{blue}{Lcom/test/Main;->normal(Ljava/lang/String;)V}@>
  invoke-virtual { p0, v1 }, \
  <@\ \ Lcom/ecspride/Main;->bytecodeTamper(I)V@>
  add-int/lit8 v1, v1, 1
  goto :L0
  :L1
  return-void
.end method
\end{lstlisting}

\vspace{-5pt}

\begin{lstlisting}[caption={This smali code represents the method \texttt{leak} after the first execution of method \texttt{bytecodeTamper}.},label={lst:fe}, language=Ant]
.method public leak()V
  <@\textcolor{blue}{const-string v0, "non-sensitive data"} @>
  <@\textcolor{blue}{nop} @>
  <@\textcolor{blue}{nop} @>
  const/4 v1, 0
  :L0
  const/4 v2, 2
  if-ge v1, v2, :L1
  <@\textcolor{red}{invoke-virtual { p0, v0 }, \textbackslash}@>
  <@\ \ \textcolor{red}{Lcom/test/Main;->sink(Ljava/lang/String;)V}@>
  invoke-virtual { p0, v1 }, \
  <@\ \ Lcom/ecspride/Main;->bytecodeTamper(I)V@>
  add-int/lit8 v1, v1, 1
  goto :L0
  :L1
  return-void
.end method
\end{lstlisting}


==> paragraphs/threat-model.tex <==
\section{Threat Model and Assumptions}
\label{sec:threat-model}

In our system, we treat all application developers with potentially malicious purpose. They 
can use sophisticated technology such as packing to evade static analysis 
tools. 
%We make no assumption in regard to the mechanism by which the malicious code is packed.
%The application may be packed by commercial packers or self-defined algorithms. 
Moreover, the application may contain
self-modifying code, which manipulates its bytecode at runtime. 
We make no assumption on how or when these technologies are used, but we assume that the malicious
code in an application is executed at some point.
%For the packed applications, we assume that the malicious code is executed at some point, and the code 
%can be packed again after its execution.

As our system runs inside ART, we assume that the Android operating system is not
compromised and applications cannot gain root privilege during 
their execution. Moreover, as the revealed result is fed to static analysis tools,
we assume that the static analysis tools function correctly.

